Are We Ready for Real-Time LiDAR Semantic Segmentation in Autonomous Driving?

Within a perception framework for autonomous mobile and robotic systems, semantic analysis of 3D point clouds typically generated by LiDARs is key to numerous applications, such as object detection and recognition, and scene reconstruction. Scene semantic segmentation can be achieved by directly integrating 3D spatial data with specialized deep neural networks. Although this type of data provides rich geometric information regarding the surrounding environment, it also presents numerous challenges: its unstructured and sparse nature, its unpredictable size, and its demanding computational requirements. These characteristics hinder the real-time semantic analysis, particularly on resource-constrained hardware architectures that constitute the main computational components of numerous robotic applications. Therefore, in this paper, we investigate various 3D semantic segmentation methodologies and analyze their performance and capabilities for resource-constrained inference on embedded NVIDIA Jetson platforms. We evaluate them for a fair comparison through a standardized training protocol and data augmentations, providing benchmark results on the Jetson AGX Orin and AGX Xavier series for two large-scale outdoor datasets: SemanticKITTI and nuScenes.

==> sec/3_methodology.tex <==
\section{METHODOLOGY}
\label{sec:methodology}
We aim to provide a benchmark analysis for state-of-the-art semantic segmentation methods on embedded systems, identify bottlenecks and shortcomings of different methodologies on such computing architectures, study the trade-off between prediction accuracy and computational cost, provide a fair comparative analysis of different neural networks on several datasets, and extract valuable information on network design choices for embedded semantic segmentation.

% \subsection{Datasets}
% \label{subsec:datasets}
% % Numerous studies, including~\cite{ullah2020benchmarkingclassification, qian2022pointnext}, target 3D object-based synthetic datasets such as ModelNet40~\cite{zhirong20153dshapenets} for benchmarks and point cloud analysis, typically for object classification tasks.
% We focus on the semantic segmentation task for real-time applications\textemdash that is mobile autonomous and robotic systems; therefore, we target two large-scale datasets to study outdoor semantic segmentation on SemanticKITTI~\cite{behley2019semantickitti} and nuScenes~\cite{caesar2020nuscenes} for the challenging outdoor perception application of autonomous vehicles in real-time. The point cloud acquisition sensors for those outdoor datasets are two different LiDAR scanners (velodyne HDL-64E and HDL-32E respectively)  that provide different point cloud characteristics in terms of density/sparsity and total number of points. 
% We also target indoor mobile systems that require perceiving indoor scenes in real-time; hence we select ScanNetv2~\cite{dai2017scannet} that is collected using an RGB-D sensor, which further generalizes our validation approach.

% ~\cite{zhirong20153dshapenets}

%~\cite{ullah2020benchmarkingclassification, ma2022pointmlp, qian2022pointnext}
%We provide a brief description of each considered dataset as follows:
 % \textbf{SemanticKITTI.}  This dataset showcases urban outdoor environments (i.e., city traffic, residential blocks, highways) captured with a Velodyne HDL-64E LiDAR covering the full 360\degree\ Field-of-View. We follow the same division of its 22 sequences, and only work with sequences 00 to 10 designated for training except for the 8$^{\text{th}}$ used for validation.
 
 % and sequences 11 to 21 as test set.
 
 % In total, SemanticKITTI offers for training 23,201 complete 3D scans and for testing 20,351 ones, and provides point-wise annotations for 28 classes of which 25 are used to evaluate methods on semantic scene understanding.

 % \textbf{nuScenes.} It was the pioneering outdoor dataset that encompasses a comprehensive autonomous vehicle sensor suite consisting including a Velodyne HDL-32E LiDAR, offering a complete 360\degree\ FoV while driving in Boston and Singapore, two cities very well known for their dense traffic and challenging driving situations. 
 
 % nuScenes offers 1000 scenes of 20s duration each, providing 40,157 scans of 1.4 billion points in total all annotated with 32 classes, 16 of them used for evaluation.
 
 % \textbf{ScanNet.} When it comes to RGB-D semantic scene understanding, ScanNet provides 1,513 scans of more than 707 distinct indoor environments. The acquisition sensor used is Structure sensor an RGB-D sensor with a design similar to the Microsoft Kinect v1. 

 % little data was available prior to ScanNet, with only some datasets covering small range of scene views and limited semantic annotations. ScanNet addressed this issue, by
 % Additionally, voxel-wise annotations are provided for 20 classes all used for evaluation.
% \subsection{Selected 3D Neural Networks}
% \label{subsec:neuralnetworks}
% Among the state-of-the-art 3D semantic segmentation methods, we will select few well-performing ones that belong to the different categories presented in \cref{sec:relatedwork}:

% From the projection-based methods, SalsaNext~\cite{cortinhal2020salsanext} provides a good trade-off between segmentation accuracy and runtime when compared to other methods from this category; it is developed based on the LiDAR range view image obtained from the spherical projection~\cite{milioto2019rangenet++}, which is the baseline of all projection-based methods.

% We also consider WaffleIron~\cite{puy2023waffleiron} from the point-based methods, a recent backbone that solely relies on dense 2D convolutions and generic MLPs, making it less complicated in terms of design choices than numerous other methods. It also proved to be among the best performing in this category on the large-scale SemanticKITTI~\cite{behley2019semantickitti} and  nuScenes~\cite{caesar2020nuscenes}. Therefore, it is worth investigating on embedded systems.

% From the sparse convolution-based methods, Minkowski~\cite{choy2019minkowski} proposed the most generalized high-dimensional sparse tensor computations that leverage the sparsity in point clouds to lower memory consumption and accelerate inference, while considering 3D voxels instead of 2D ones that suffer from loss in geometry and topology. Many other methods build on top of Minkowski~\cite{cheng2021(af)2-s3net, tang2020spvnas}, thereby making it suitable for benchmarking. For example, SPVConv~\cite{tang2020spvnas} incorporated the sparse 3D convolution with a point-wise MLP to subsequently fuse the extracted features from both levels together, to better classify small instances and increase the overall accuracy. This fusion-based method will also be investigated.

% For each selected neural network, we evaluate its baseline model, and create another variant that is lighter in order to achieve performance gains on embedded systems, and assess the variant's capability of being deployed in resource-constrained platforms.
% Additionally, it supports custom kernel shapes and is not limited to specific kernel dimensions

% \subsection{Embedded Computing Architectures}
% \label{subsec:embeddedsystems}
% Although deep neural networks are credible for solving several complex tasks, they are computationally cumbersome in terms of resources and time required to perform the involved operations. Therefore, substantial work has been invested in the context of effectively implementing computationally expensive algorithms on different specialized hardware architectures. \cite{dhilleswararao2022surveyhardwarearchitectures} provides a comparative study between different hardware architectures mainly the graphics processing unit (GPU), the field-programmable gate array (FPGA), and the application specific integrated circuit (ASIC), based on factors such as power consumption
% % , area (proportion of silicon required depending on the size of the on-chip memory)
% and throughput. It has been observed on several applications involving image classification, and object detection
% % , speech recognition, and natural language processing 
% that CPU- and GPU-based architectures consume more power than FPGA and ASIC counterparts, but offer an overall higher throughput. Similarly, \cite{hu2022surveycnnaccelerators} presents a survey on CNNs
% % that are widely used in numerous applications (including semantic segmentation)
% on the same hardware architectures and state that GPU-based ones are the most adapted at the cost of higher energy consumption, FPGA-based ones are inferior in performance but offer high flexibility and low energy usage, and finally ASIC-based ones are highly inflexible due to their targeted designs. 
% \begin{table}[b!]
% \caption{The targeted Jetson platforms specifications.}
% \label{tab:nvidia_jetson}
% \centering
% \resizebox{0.47\textwidth}{!}{
% \begin{tabular}{|c|c|c|}
% \hline
% \textbf{Version} & \textbf{Jetson AGX Orin} & \textbf{Jetson AGX Xavier} \\
% \hline
% %\tablefootnote{https://www.nvidia.com/en-us/autonomous-machines/embedded-systems/jetson-orin/}
% %\tablefootnote{https://www.nvidia.com/en-us/autonomous-machines/embedded-systems/jetson-agx-xavier/}
% \textbf{Performance} & 275 TOPS & 32 TOPS \\
% \hline

% \textbf{GPU} & \begin{tabular}{@{}c@{}}2048-core NVIDIA \\ Ampere architecture GPU \\ with 64 Tensor Cores\end{tabular} & \begin{tabular}{@{}c@{}}512-core NVIDIA \\ Volta architecture GPU \\ with 64 Tensor Cores\end{tabular} \\
% \hline

% \textbf{CPU} & \begin{tabular}{@{}c@{}}12-core Arm® \\ Cortex®-A78AE v8.2 64-bit \\ CPU 3MB L2 + 6MB L3\end{tabular} & \begin{tabular}{@{}c@{}}8-core NVIDIA Carmel \\ Arm®v8.2 64-bit CPU \\ 8MB L2 + 4MB L3\end{tabular} \\
% \hline

% \textbf{Memory} & 64 GB & 32 - 64 GB \\
% \hline

% \textbf{Power} & 15W - 60W & 10W - 30W \\
% \hline

% \end{tabular}
% }

% \end{table}
% Therefore, it is not straightforward to conclude that certain architectures are superior to others.
% % since this depends on the target application and the system requirements. 
% But since most robotic and autonomous systems adopt GPU-based architectures, and 3D perception models are highly in demand for such systems, we consider GPU-based computing platforms towards embedding well-performing 3D semantic segmentation models. More specifically, we target two Jetson platforms, the AGX Orin, and AGX Xavier presented in \cref{tab:nvidia_jetson}, since they offer a good compromise among performance, efficiency, and cost. They also offer a varying range of performance, memory, and power, thereby making them suitable for benchmarking.


% \subsection{OpenNeuralPC Framework}
% Numerous technical challenges arise when attempting to directly implement a Python or Conda environment on the Jetson platforms. These challenges originate from the discrepancies in configurations, supported environments, packages and software dependencies in between the Jetson embedded modules and the workstation machines that all methods rely on for training and inference. Consequently, deploying various neural network models on embedded systems becomes a complex task.

% To overcome these challenges, we create a PyTorch-based framework\textemdash that is \textbf{OpenNeuralPC}\textemdash that can be deployed directly to Jetson platforms without complications, and that easily integrates different neural networks for training, validating, and testing on different datasets. OpenNeuralPC adeptly resolves the following complexities: \\
% \indent
% \textbf{Framework compatibility}: Popular deep learning frameworks such as TensorFlow and PyTorch have limited support and are resource-intensive on embedded platforms. OpenNeuralPC adopts a JetPack optimized tensor library for deep learning creating a lightweight Pytorch-based framework that is compatible with such systems. \\
% \indent
% \textbf{Cross-platform portability}: Ensuring seamless deployment across various platforms with minimal or no modifications is a challenging task due to variations in computing architectures, operating systems, and available libraries. OpenNeuralPC is configured to run efficiently and smoothly on Jetson embedded and desktop machines (tested on AGX Orin, AGX Xavier, Nano, RTX 4090 and RTX 3090). \\
% \indent
% \textbf{Hardware accelerators}:  Embedded systems leverage hardware accelerators such as Programmable Vision and Deep Learning Accelerators (PVA \& DLA), TensorRT library that optimizes inference performance on NVIDIA Jetson, as well as Tensor Cores to enable mixed-precision computing. OpenNeuralPC supports such accelerators and optimizes the models accordingly to significantly enhance performance on those resource-constrained systems. \\
% \indent
% \textbf{Profiling}:  Development and profiling challenges on embedded systems arise due to limited debugging capabilities compared to desktop environments, making it challenging to identify and rectify issues during model deployment. OpenNeuralPC integrates various tools and profilers crucial for assessments in embedded platforms. \\
% \indent
% Additionally, OpenNeuralPC enables the reproduction of any 3D point cloud semantic scene understanding model from all four categories presented \cref{subsec:semanticsegmentationrelatedwork}, as opposed to OpenPoints~\cite{qian2022pointnext}, an engine that only supports the reproduction of point-based methods. It also integrates various choices of training protocol: optimizer, scheduler, loss function, batch size, number of epochs, and set of data augmentations. As observed in~\cite{qian2022pointnext}, a significant improvement in performance can be attributed to the training methods, and OpenNeuralPC employs such enhanced techniques and enables an aligned training for all the considered models resulting in a fair network comparison. Therefore, our framework offers benefits on different aspects, namely the scalability, fair benchmarking, and deployability to Jetson embedded platforms.


% \underline{scalability} as it supports and integrates any neural network for 3D point cloud semantic scene understanding from any category and on several large scale datasets;
% \underline{reproducibility} as it supports training and reproducing a model with various choices of training protocol: optimizer, scheduler, loss function, batch size, number of epochs, and set of data augmentations;
% \underline{fair benchmarking} as stated in~\cite{qian2022pointnext}, it is observed that a significant improvement in the performance can be attributed to the training methods, and OpenNeuralPC employs these enhanced training techniques, enables an aligned training for all the considered models and, hence, offers a fair comparison in terms of accuracy rather than considering the initially reported values; and finally it is
% % \underline{ease of use} since it can easily build a new model or integrate a new dataset, or vary the training protocol and data augmentations for the 3D semantic segmentation task;
% \underline{embeddable} since it can be directly deployed to Jetson platforms and run smoothly without complications. 
% % and finally provided as \underline{open source} for public and community use.

